Bounds on the Achievable Rate of Noisy feedback Gaussian Channels under Linear Feedback Coding Scheme

In this paper, we investigate the additive Gaussian noise channel with noisy feedback. We consider the setup of linear coding of the feedback information and Gaussian signaling of the message (i.e. Cover-Pombra Scheme). Then, we derive the upper and lower bounds on the largest achievable rate for this setup. We show that these two bounds can be obtained by solving two convex optimization problems. Finally, we present some simulations and discussion.

==> intro_ISIT11.tex <==
\indent The study of the additive Gaussian noise channel with feedback has been a hot research topic for decades. So far, a large body of work has looked at the ideal feedback case and obtained many notable results \cite{Schalkwijk66,Omura68,Massey1990,cover89,Kim10}. As an illustration, it is known that noiseless feedback improves the error exponent and reduces the coding complexity. However, only few papers have studied channels with noisy feedback and many open problems still exist. Literature on noisy feedback problems can be largely classified into two categories. The first category studies the usefulness of noisy feedback by investigating reliability functions and error exponents \cite{Kim07},\cite{Love_arxiv}. The second focuses on the derivation of coding schemes based on the well-known Schalkwijk-Kailath scheme. We refer interested readers to \cite{Omura68,Lavenberg71,Martins08,Chance10,Kumar} for details.\\
\indent In this paper, we investigate the behavior of the largest achievable rate of the additive Gaussian noise channel with noisy feedback. Based on Cover-Pombra Scheme (i.e. linear coding of feedback information and Gaussian signaling), we derive informative upper and lower bounds on the largest achievable rate. This upper bound outperforms the bound presented in \cite{Love10}, especially, in the case of having small feedback noise. The lower bound shows the enhancement, in terms of the achievable rate, by exploiting the noisy feedback link. Additionally, the derived bounds provide insight on how the noisy feedback channel behaves with respect to the feedback noise.\\
\indent The paper is organized as follows. In Section \ref{sec_pre}, we introduce some important definitions and lemmas, which are used throughout the paper. In Section III, we introduce the signal model of the noisy feedback channel and then derive the formula of the achievable rate. In Section \ref{sec_upper} and \ref{sec_lower}, we derive an upper bound and a lower bound on the largest achievable rate, respectively. We present some simulation results and discussion in Section \ref{sec_simu} and conclude the paper in Section \ref{sec_conclude}.\\
\indent Notations: Uppercase and corresponding lowercase letters $(e.g. Y,Z,y,z)$ denotes random variables and realizations, respectively. $x^n$ represents the vector $[x_1,x_2,\cdots,x_n]^T$ and $x^0=\emptyset$. $\mathbf{I}_n$ represents an $n\times n$ identity matrix. $\mathbf{K}_n>0$ ($\mathbf{K}_n\geq 0$) denotes that the $n\times n$ matrix $\mathbf{K}_n$ is positive definite (semi-definite). $log$ denotes the logarithm base $2$ and $0\log0=0$. The expectation operator over $X$ is presented as $\mathbb{E}(X)$. 
